Smoothed analysis for low-rank solutions to semidefinite programs in quadratic penalty form

Semidefinite programs (SDP) are important in learning and combinatorial optimization with numerous applications. In pursuit of low-rank solutions and low complexity algorithms, we consider the Burer--Monteiro factorization approach for solving SDPs. We show that all approximate local optima are global optima for the penalty formulation of appropriately rank-constrained SDPs as long as the number of constraints scales sub-quadratically with the desired rank of the optimal solution. Our result is based on a simple penalty function formulation of the rank-constrained SDP along with a smoothed analysis to avoid worst-case cost matrices. We particularize our results to two applications, namely, Max-Cut and matrix completion.

==> app_pd_reorganized.tex <==
\section{Proofs of results in Section~\ref{sec:pd}}

==> counterexample_constrained.tex <==
\section{Counterexample for the constrained case}
Fix dimension $n$, number of constraints $m = n-1$ and rank $k= n-2$. Define the following matrices:
\begin{align*}
	C &= \begin{bmatrix}
	\eye_{n-2 \times n-2}	&	\ones_{n-2 \times 2} \\
	\ones_{2 \times n-2}	&	\begin{array}{cc}
	2n	& 0 \\ 0 & 0
	\end{array}
	\end{bmatrix},
	\mbox{ and } \\
	A_i &= \begin{bmatrix}
	\zeros_{n-2\times n-2} & \begin{array}{c}
	\zeros_{i-1 \times 2} \\ \ones_{1 \times 2} \\ \zeros_{n-2-i \times 2}
	\end{array} \\
	\begin{array}{ccc}
	\zeros_{2 \times i-1} & \ones_{2 \times 1} & \zeros_{2 \times n-2-i } \end{array} & \begin{array}{cc}
	0	& 0 \\ 0 & 1
	\end{array}
	\end{bmatrix}, \mbox{ for } i = 1,\cdots, n-2,
\end{align*}
where $\zeros, \ones, \eye$ represent all zeros, all ones and identity matrix respectively of appropriate sizes. The counter example problem is

\begin{align}
	&\min_{U \in \R^{n\times k}} \trace{\trans{U} C U} \nonumber \\
	& \mbox{ s.t. } \trace{\trans{U} A_i U} = 0 \mbox{ for } i = 1,\cdots, n-2 \nonumber \\
	&\qquad \trace{U \trans{U}} = n-2. \label{eq:counter-constrained}
\end{align}

The following lemma shows that on the constraint manifold, $U = \eye_{n \times k}$ is a suboptimal second order optimal point.
\begin{lemma}
Let $k=n-2$, then $U = \eye_{n \times k}$ satisfies second order optimality on the constraint manifold and is suboptimal for problem \eqref{eq:counter-constrained}. 
\end{lemma}
\begin{proof}

\noindent \textbf{Suboptimality of $U$}: For $U = \eye_{n \times k}$, $UU^T$ is a $n\times n$ matrix with a $k \times k$ Identity block. Since the first $n-2$ constraints have $0$ in the top $k \times k$ block, we get that $\ip{A_i}{UU^T}=0, 1 \leq i \leq n-2$. Also $\trace{UU^T}$ is $k=n-2$. Hence, $UU^T$ is a feasible point for the above SDP. 

Computing the objective value of~\eqref{eq:counter-constrained} at $U$, we see that it is equal to $n-2$. Define $w \defeq \trans{\begin{bmatrix}
\ones_{1\times n-2} & 0 & -1
\end{bmatrix}}$. Consider now a different matrix $\displaystyle X_0 \defeq \frac{n-2}{n} \left(w \trans{w} + \begin{bmatrix} \zeros_{n-1 \times n-1} & \zeros_{n-1 \times 1} \\ \zeros_{1 \times n-1} & 1 \end{bmatrix}\right)$. It is easy to see that $X_0$ is PSD and satisfies all the constraints in~\eqref{eq:counter-constrained}. Furthermore, we see that the objective value at $X_0$, $$\displaystyle \ip{C}{X_0} = \frac{n-2}{n} \cdot \trans{w}Cw = \frac{(n-2)^2}{n} < n-2 =\ip{C}{UU^T}.$$ This proves that $UU^T$ is suboptimal to the above SDP.\\

\noindent	\textbf{Second order optimality:} The space orthogonal to the constraint manifold at $U$ is given by $\displaystyle \Ps \defeq \linspan{U,  A_i U; i\in[n-2]}$. The first order optimality conditions are satisfied since the gradient of the objective, $CU = U + \sum_{i=1}^{n-2} A_i U,$ is in $\Ps$, and is orthogonal to the constraint manifold. 


We will now show that for any perturbation along the tangent space at $U$, the objective value strictly increases, thereby showing that $U$ satisfies second order optimality conditions. Any perturbation $\DelU$ in the tangent space at $U$, by definition is orthogonal to $\Ps$ ($\DelU \perp \Ps$). Let $\DelU$ be given by $$\DelU \defeq \begin{bmatrix} {\DelUbar}_{n-2 \times n-2} \\ \Delu_1 \; \Delu_2 \; \cdots \; \Delu_{n-2} \end{bmatrix},$$ where each $\Delu_i$ is a $2\times1$ vector. Since $\Delu \perp A_i U$ for every $i$, we see that $\trans{\ones_{2\times 1}}\Delu_i = 0$ for every $i \in [n-2]$. Hence for any point $U+\DelU$ on the constraint manifold,
\begin{align}
	&\trace{\trans{\left(U + \DelU\right)} A_i \left(U + \DelU\right)} = \trace{\trans{U} A_i U} \nonumber \\
	\Rightarrow & 2 \trace{\trans{\DelU} A_i U} + \trace{\trans{\DelU} A_i \DelU} = 0. \label{eq:constraints-unchanged}
\end{align} Similarly the $\trace{UU^T}=n-2$ constraint gives us, $2\trace{\trans{\DelU}U}+\trace{\trans{\DelU} \DelU}=0$.

Further, the change in objective value is,
\begin{align*}
	\trace{\trans{\left(U + \DelU \right)} C \left(U + \DelU \right)} - \trace{\trans{U}C U} &= 2 \trace{\trans{\DelU} C U} + \trace{\trans{\DelU} C \DelU} \\
	&= 2 \trace{\trans{\DelU} \left(U + \sum_i A_i U\right) } + \trace{\trans{\DelU} C \DelU} \\	
	&\stackrel{\zeta_1}{=} -\trace{\trans{\DelU} \left(\DelU + \sum_i A_i \DelU\right) } + \trace{\trans{\DelU} C \DelU} \\	
	&= \trace{\trans{\DelU} \left(C - \sum_i A_i - \eye \right) \DelU} \\
	&= \sum_{i=1}^{n-2} \trans{\Delu}_i D \Delu_i,
\end{align*}
where $D\defeq \begin{bmatrix} 2n-1 & 0 \\ 0 & -(n-1) \end{bmatrix}$. $\zeta_1$ follows from \eqref{eq:constraints-unchanged}. Since all perturbations in the tangential space satisfy $\trans{\ones_{2 \times 1}}\Delu_i=0$, we see that $\Delu_i \in \linspan{\begin{bmatrix}
	1 \\ -1
	\end{bmatrix}}$. Since $\begin{bmatrix}
1 & -1
\end{bmatrix} D \begin{bmatrix}
1 \\ -1
\end{bmatrix} = n > 0$, this shows that objective value strictly increases for any perturbation along the tangential space at $U$.
\end{proof}
